Visual-O1: Understanding Ambiguous Instructions via Multi-modal Multi-turn Chain-of-thoughts Reasoning

As large-scale models evolve, language instructions are increasingly utilized in multi-modal tasks. Due to human language habits, these instructions often contain ambiguities in real-world scenarios, necessitating the integration of visual context or common sense for accurate interpretation. However, even highly intelligent large models exhibit significant performance limitations on ambiguous instructions, where weak reasoning abilities of disambiguation can lead to catastrophic errors. To address this issue, this paper proposes Visual-O1, a multi-modal multi-turn chain-of-thought reasoning framework. It simulates human multi-modal multi-turn reasoning, providing instantial experience for highly intelligent models or empirical experience for generally intelligent models to understand ambiguous instructions. Unlike traditional methods that require models to possess high intelligence to understand long texts or perform lengthy complex reasoning, our framework does not significantly increase computational overhead and is more general and effective, even for generally intelligent models. Experiments show that our method not only significantly enhances the performance of models of different intelligence levels on ambiguous instructions but also improves their performance on general datasets. Our work highlights the potential of artificial intelligence to work like humans in real-world scenarios with uncertainty and ambiguity. We will release our data and code.

==> Content/04_Experiment_bak.tex <==
\section{Experiments}

\subsection{Experimental Setup}

To verify the effectiveness of our method, we evaluate three typical multimodal scenarios: visual question answering (VQA), referring image segmentation (RIS), and visual language navigation (VLN). We use three state-of-the-art instruction-based models for validation for each of these tasks.
We use LLaVA-1.5, LISA, and VLN-SIG for VQA, RIS, and VLN task.

We set up three extra ambiguous datasets for VQA, RIS, and VLN task that only contain ambiguous instructions through manual filtering or refinement. We conduct experiments on all three tasks and ensured that all models are under the same settings. For more details, please refer to the \textbf{Appendix} \ref{edata}. 

\subsection{Overall Results}

\begin{table}[t!]
\caption{\textbf{Overall results on Ambigous-RIS.} Compared with LISA, which can hardly correctly segment any targets, the accuracy can be greatly improved after combining with Vigor. The improvement is statistically significant with $p < 0.01$ under $t$-test.}
\vskip -0.05in
\label{tab:overall_ris}
\setlength{\tabcolsep}{2.6mm}
% \vskip -0.2in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccc}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{LMM} & \multirow{2}{*}{Disambiguation} & \multicolumn{2}{c}{Ambigous-RIS} \\
\cmidrule{4-5} & & & gIoU & cIoU \\
\midrule
LISA \citep{lai2023lisa} & LLaVA & - & $0.0237$ & $0.0272$\\
LISA + Vigor & LLaVA & LLaVA & $\mathbf{0.1088 (+359.07\%)}$ & $\mathbf{0.1209 (+344.49\%)}$\\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.15in
\end{table}

\begin{table}[t!]
\caption{\textbf{Overall results on Ambigous-VQA.} A similar phenomenon was also observed in VQA, that the performance of ambiguous instructions will be significantly improved after LLaVA is combined with Vigor. The improvement is statistically significant with $p < 0.01$ under $t$-test.}
\setlength{\tabcolsep}{2.7mm}
\vskip -0.05in
\label{tab:overall_vqa}
% \vskip -0.2in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccc}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{LMM} & \multirow{2}{*}{Disambiguation}  & \multicolumn{2}{c}{Ambigous-VQA} \\
\cmidrule{4-5} & & & Acc & BLEU-1 \\
\midrule
LLaVA \citep{liu2024improved} & LLaVA & - & $4.98$ & $0.2150$ \\
LLaVA + Vigor & LLaVA & LLaVA & $\mathbf{27.43 (+450.80\%)}$ & $\mathbf{0.4103 (+90.84\%)}$\\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.15in
\end{table}

\begin{table}[t!]
\caption{\textbf{Overall results on Ambigous-VLN.} On VLN, Vigor can also improve the effects of ambiguous instructions. The improvement is statistically significant with $p < 0.01$ under $t$-test.}
\setlength{\tabcolsep}{4.5mm}
\vskip -0.05in
\label{tab:overall_vln}
% \vskip -0.2in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lccc}
\toprule
\multirow{2}{*}{Model} & \multicolumn{3}{c}{Ambigous-VLN} \\
\cmidrule{2-4} & SR & SPL & Navi Error \\
\midrule
VLN-SIG \citep{li2023improving} & $4.72$ & $4.59$ & $7.95$\\
VLN-SIG + Vigor  & $\mathbf{26.42 (+459.75\%)}$ & $\mathbf{22.66 (+393.68\%)}$ & $\mathbf{5.99 (-24.65\%)}$\\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.15in
\end{table}

As shown in Table \ref{tab:overall_ris}, \ref{tab:overall_vqa}, and \ref{tab:overall_vln}, we observe that the original models all produce inferior results on the three different tasks of VQA, RIS, and VLN. This suggests that existing methods are susceptible to ambiguous instructions and struggle to understand instructions that require combining visual context correctly.

However, after integrating Vigor, all tasks significantly improved by more than $100\%$. This means that existing methods have the potential to understand ambiguous instructions but need the correct guidance. It is worth noting that in VQA, LISA is trained based on LLaVA, so we did not introduce additional models or data for VQA and RIS. This means that we can effectively alleviate the problem of different models understanding ambiguous instructions on different tasks without incurring additional costs. For comparisons with baseline models, kindly refer to Section \ref{general}.

\subsection{Generalized Studies}

\paragraph{Non-ambiguous Data}
\label{general}
\begin{table}[t!]
\caption{\textbf{Results on general RIS.} On the non-ambiguous general dataset, Vigor also showed effectiveness, significantly improving the performance of the model. "-" indicates that the original paper did not report the results.}
\label{tab:ger_ris}
% \vskip -0.2in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcc}
\toprule
\multirow{2}{*}{Model} & \multicolumn{2}{c}{RIS} \\
\cmidrule{2-3} & gIoU & cIoU \\
\midrule
OVSeg \citep{liang2023open} & $0.0418$ & $0.0778$ \\
Ref-Diff \citep{ni2023ref} & $0.3301 $ & $0.3140$ \\
Unified-IO \citep{lu2022unified} & $-$ & $0.4015$ \\
InstructDiffusion \citep{geng2023instructdiffusion} & $-$ & $0.3904$ \\
SoM \citep{yang2023set} & $0.3507$ & $0.4154$ \\
% GRES & $\times$ & $\times$ \\
% X-Decoder & $\times$ & $\times$ \\
%SAM-CLIP & $0.2684$ & $0.2606$ \\
%GLOBAL-LOCAL CLIP & $0.2784$ & $0.2583$ \\
%CROPPING & $0.2646$ & $0.2393$ \\
%REGION TOKEN & $0.2537$ & $0.2346$ \\
LISA \citep{lai2023lisa} & $0.4654$ & $0.4721$ \\
LISA + Vigor & $\mathbf{0.4806}$ & $\mathbf{0.4745}$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.15in
\end{table}

\begin{table}[t!]
\caption{\textbf{Results on general VQA.} Vigor significantly improves the performance of the general dataset, further proving its effectiveness. "-" indicates that the original paper did not report the results.}
\label{tab:ger_vqa}
% \vskip -0.2in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcc}
\toprule
\multirow{2}{*}{Model} & \multicolumn{2}{c}{VQA} \\
\cmidrule{2-3} & Acc & BLEU-1 \\
\midrule
BLIP2 6.7B \citep{li2023blip}  & $24.64$ & $0.3138$ \\
InstructBLIP \citep{dai2024instructblip} & $34.15$ & $0.5393$ \\
%X-InstructBLIP 7B& $34.90$ & $-$ \\
%Flamingo 9B & $28.80$ & $-$ \\
Qwen-VL-chat \citep{bai2023qwen} & $38.90$ & $-$ \\
MoE-LLaVA \citep{lin2024moe} & $35.56$ & $0.5658$ \\
Video-LLaVA \citep{lin2023video} & $48.10$ & $-$ \\
Otter \citep{li2023otter} & $50.00$ &$-$ \\
MiniGPT-v2 \citep{chen2023minigpt} & $33.68$ & $0.5507$ \\
MiniGPT-v2(chat) \citep{chen2023minigpt} & $53.66$ & $0.6816$ \\
LLaVA \citep{liu2024improved} & $54.19$ & $0.7194$ \\
LLaVA + Vigor & $\mathbf{57.38}$ & $\mathbf{0.7329}$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.15in
\end{table}

Although the ability to understand ambiguous instructions is crucial, it is also essential for the model to maintain its capability on general datasets. To verify this, we conduct experiments on the general datasets of VQA and RIS. As shown in Tables \ref{tab:ger_ris} and \ref{tab:ger_vqa}, we find that Vigor significantly enhances the understanding of ambiguous instructions and significantly improves the performance on general datasets. This is because enhancing their understanding is also beneficial even for instructions that do not contain ambiguity. This also demonstrates the generalizability of our method, which also has advantages on general datasets.

\paragraph{Various Disambiguation Models}

\begin{table}[t!]
\caption{\textbf{Generalized results on different disambiguation and downstream task models.} Vigor has shown effectiveness on different task models and different disambiguation models.}
\setlength{\tabcolsep}{2.6mm}
\label{tab:abl}
% \vskip -0.2in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccccccc}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{LMM} & \multirow{2}{*}{Disambiguation} & \multicolumn{2}{c}{Ambiguous-RIS} & &  \multicolumn{2}{c}{RIS}\\
\cmidrule{4-5}\cmidrule{7-8} & & & gIoU & cIoU & & gIoU & cIoU \\
\midrule
LISA \citep{lai2023lisa}  & LLaVA & - & $0.0237$ & $0.0272$ && $0.4704$ & $0.4859$\\
LISA + Vigor  & LLaVA & LLaVA & $0.1088$ & $0.1209$ && $0.4794$ & $0.5004$\\
LISA + Vigor  & LLaVA & GPT-4V & $\mathbf{0.1447}$ & $\mathbf{0.1351}$ && $\mathbf{0.4985}$ & $\mathbf{0.5188}$\\
\midrule
SoM \citep{yang2023set}  & GPT-4V & - & $0.0752$ & $0.1158$ && $0.3507$ & $0.4154$\\
SoM + Vigor  & GPT-4V & GPT-4V & $\mathbf{0.1143}$ &$\mathbf{0.1530}$ && $\mathbf{0.3772}$ & $\mathbf{0.4336}$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.15in
\end{table}

We set up additional experiments to explore whether Vigor is effective on different disambiguation models. As shown in Table \ref{tab:abl}, we find that on LISA, whether using LLaVA or GPT-4V as a disambiguation model, we can significantly improve its performance on ambiguous instructions while maintaining the effect on the general dataset. Furthermore, we found that GPT-4V, as a disambiguation model, can produce better results, regardless of whether it is an ambiguous or a general dataset, because GPT-4V can generate more accurate responses. However, even with a weaker LLaVA, the improvement is still significant.

\paragraph{Various Downstream Models}

How does Vigor generalize to different downstream task models? We choose two powerful but different RIS models, SoM based on GPT-4V and LISA based on LLaVA. As shown in Table \ref{tab:abl}, we observe a significant improvement, regardless of the downstream model. This proves the generalizability of our method to different downstream task models and opens up possibilities for a broader application of our method.

\subsection{Ablation Studies}

\begin{table}[t!]
\caption{\textbf{Ablation studies.} Compared to other methods, Vigor not only significantly improves the performance on ambiguous instructions without the need for additional data but also maintains good performance on the general dataset.}
\label{tab:abl2}
\setlength{\tabcolsep}{2.6mm}
% \vskip -0.2in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lccccc}
\toprule
\multirow{2}{*}{Model} & \multicolumn{2}{c}{Ambiguous-VQA} & &  \multicolumn{2}{c}{VQA}\\
\cmidrule{2-3}\cmidrule{5-6} & Acc & BLEU-1 & & Acc & BLEU-1 \\
\midrule
LLaVA + CoT \citep{wei2022chain} & $18.05$ & $0.2634$  && $39.78$ & $0.5113$ \\
%LLaVA + WaffleCLIP & $\times$ & $\times$ && $\times$ & $\times$ \\
LLaVA + FuDD \citep{esfandiarpoor2023follow} & $21.23$ & $0.3111$ && $48.37$ & $0.6454$ \\
%LLaVA + Fine-tuning \citep{liu2024improved} & $\times$ & $\times$ && $\times$ & $\times$ \\
LLaVA + Lora Fine-tuning \citep{hu2021lora} & $26.86$ & $0.3985$ && $51.48$ & $0.6863$ \\
\midrule
LLaVA + Vigor & $\mathbf{27.43}$ & $\mathbf{0.4103}$ && $\mathbf{57.38}$ & $\mathbf{0.7329}$ \\
\quad w/o Target-free Generative Optimization & $26.75$ & $0.4056$ && $55.81$ & $0.7138$ \\
\quad w/o Skipped Prompt Connection & $27.14$ & $0.4049$ && $47.59$ & $0.6589$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.15in
\end{table}

To further explore the effectiveness of Vigor, we conduct ablation experiments in the general and ambiguous VQA data in Table \ref{tab:abl2}. Target-free generative optimization is crucial for the model to understand ambiguous instructions correctly. The model's performance on ambiguous data significantly decreases without target-free generative optimization. Meanwhile, the skipped prompt connection is very important for the performance of regular data from non-ambiguous data, as the original instruction may contain important information, and the skipped prompt connection ensures the complete transmission of information. Every module of Vigor significantly improves the model's performance on different datasets.

Not only that, we also compare baseline methods for enhancing instruction understanding. We found that Chain-of-Thought (CoT) cannot effectively solve the problem of understanding ambiguous instructions, and it causes a significant decrease in the performance of regular data. We also generate additional $10,000$ data for fine-tuning LLaVA, but we found that since synthetic data cannot effectively simulate instructions, there is a significant decrease in performance on VQA. Moreover, the cost of annotation and training brought by $10,000$ data is also very high. Therefore, Vigor can effectively solve the problem of understanding ambiguous instructions and maintain the performance of the general dataset.

For further analysis of computational overhead, refer to \textbf{Appendix} \ref{comp}.

\subsection{Exploration of Vigor}

\paragraph{Efficiency of Tuning}

\begin{table}[t!]
\caption{\textbf{Efficiency of tuning in Vigor.} Compared to human-designed prompts, the prompts optimized by Vigor achieve better performance, and each module has shown corresponding effects.}
\label{tab:tun}
% \vskip -0.2in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcc}
\toprule
\multirow{2}{*}{Model} & \multicolumn{2}{c}{VQA} \\
\cmidrule{2-3} & Acc & BLEU-1 \\
\midrule
Human-designed & $54.99$ & $0.7073$ \\
LLaVA + Vigor & $\mathbf{57.38}$ & $\mathbf{0.7329}$ \\
\quad w/o Multi-epochs & $55.20$ & $0.7033$ \\
\quad w/o Multi-samples & $55.75$ & $0.7092$ \\
\quad w/o Visual Contexts & $55.90$ & $0.7143$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.15in
\end{table}

We design additional validation experiments further to prove the effectiveness of Vigor's optimization process. We invite $10$ volunteers to manually design disambiguation prompts, which are used as benchmarks for ten tests and averaged. As shown in Table \ref{tab:tun}, manually designed prompts are significantly weaker than automatically optimized prompts, proving the rationality of Vigor's design. Moreover, we further verify whether Vigor's design details are effective. We find that without multi-epochs, \textit{i.e.}, only allowing optimization once in Vigor's optimization, significantly reducing the score. Without multi-samples, \textit{i.e.}, only allowing optimization for the same sample will lead to overfitting and cannot optimize effectively. Without visual contexts, Vigor's optimization ability will also decline, as it helps the optimizer determine the current state of optimization. By avoiding all the above problems, Vigor demonstrate excellent capabilities.

\paragraph{Fluctuations of Tuning}

\begin{table}[t!]
\caption{\textbf{Fluctuations of tuning in Vigor.} Optimization can significantly improve the performance of Vigor. As the optimization progresses, Vigor will achieve better results. Like machine learning, Vigor will also perform best when the optimization reaches a certain epoch.}
\label{tab:flu}
% \vskip -0.2in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcc}
\toprule
\multirow{2}{*}{Optimization Epochs} & \multicolumn{2}{c}{VQA} \\
\cmidrule{2-3} & Acc & BLEU-1 \\
\midrule
No Optimization & $54.25$ & $0.7076$ \\
Epoch 1 & $55.87$ & $0.7190$ \\
Epoch 2 & $54.16$ & $0.7049$ \\
Epoch 3 & $\mathbf{57.38}$ & $\mathbf{0.7329}$ \\
Epoch 4 & $55.27$ & $0.7147$ \\
Epoch 5 & $55.56$ & $0.7167$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.15in
\end{table}

We also show the relationship between the optimization process of Vigor and Epoch in Table \ref{tab:flu}. The score is the lowest without optimization, even lower than the manually designed prompts. However, with the optimization progress, the performance gradually grows and falls again after reaching the peak. We observe that Vigor has a trend similar to deep learning. The performance begins to grow in the early stage of learning, but the performance decreases due to overfitting after reaching a particular stage.

For an extra demonstration of learnable prompts, refer to \textbf{Appendix} \ref{eexp}.

\subsection{Case Studies}

\begin{figure}[h]
	\centering
	\includegraphics[width=14cm]{Figure/case_ris.pdf}
 %\vskip -0.15in
	\caption{\textbf{Case studies on RIS.} Our approach aids the model in understanding ambiguous instructions by incorporating Vigor, which significantly improves the accuracy of instructions, thus enabling more effective segmentation of the target.}
	\label{fig:ris}
 \vskip -0.10in
\end{figure}

How does our approach help the model better understand ambiguous instructions? To dig deeper into this question, we visualize the results of RIS. We find that ambiguous instructions are widespread in the data and often not easily detected by humans, but it can seriously impact the model. After incorporating Vigor, the accuracy of instructions has significantly improved, yielding more effective results. As shown in the first set of examples, the original instruction can describe most of the bears in the whole image because each bear has a deviation in angle. However, when combined with the image, it is found that only one bear satisfies both the turning and the slight deviation, and Vigor successfully infers this and provides an accurate description so that the task model can accurately segment the target. In the second example, the segmentation model is influenced by the word "\texttt{reading}" and incorrectly segments the people in the picture. At the same time, Vigor accurately describes that this is a bus displaying the "\texttt{reading station}" and even provides additional information to help the segmentation model locate the target. In the third example, the instruction has a grammatical problem and cannot accurately express the position of the bottle. However, when combined with Vigor, the instruction is transformed into a more accurate form, allowing the model to locate the target easily. In the fourth example, the model does not understand that 1 o'clock is a position and, therefore, cannot select the correct object, but Vigor transforms it into a clearer description, making location possible.

For more examples on VQA and VLN, please see \textbf{Appendix} \ref{ecase}.

